Evaluating Distributional Distortion in Neural Language Modeling

A fundamental characteristic of natural language is the high rate at which speakers produce novel expressions. Because of this novelty, a heavy-tail of rare events accounts for a significant amount of the total probability mass of distributions in language (Baayen, 2001). Standard language modeling metrics such as perplexity quantify the performance of language models (LM) in aggregate. As a result, we have relatively little understanding of whether neural LMs accurately estimate the probability of sequences in this heavy-tail of rare events. To address this gap, we develop a controlled evaluation scheme which uses generative models trained on natural data as artificial languages from which we can exactly compute sequence probabilities. Training LMs on generations from these artificial languages, we compare the sequence-level probability estimates given by LMs to the true probabilities in the target language. Our experiments reveal that LSTM and Transformer language models (i) systematically underestimate the probability of sequences drawn from the target language, and (ii) do so more severely for less-probable sequences. Investigating where this probability mass went, (iii) we find that LMs tend to overestimate the probability of ill formed (perturbed) sequences. In addition, we find that this underestimation behaviour (iv) is weakened, but not eliminated by greater amounts of training data, and (v) is exacerbated for target distributions with lower entropy.

==> LMs and Syntactic Complexity/SEC_background_alex.tex <==
We begin by briefly characterizing why distributions with a large
number of rare events (LNRE) emerge in natural language, and why these
events pose challenges for LMs. Furthermore, we motivate the need for
instance-level evaluation when dealing with a large number of rare
events.

\paragraph{Productivity}
In the context of language production, a language user has the ability
to produce, at any given point in their linguistic lifespan, an
utterance which they have never produced before. This creativity is
the result of the generative property of \textsl{productivity}, which
states that on the basis of finite linguistic experience, a language
user can produce and comprehend an unbounded number of grammatically
acceptable utterances \citep{chomsky1975logical}. Productive processes
induce a distribution which places non-zero probability on unseen
events at all
  practical sample sizes. Because of this property,
many of the distributions in natural language---particularly the
distribution over the sequences of a language---are characterized by a
heavy-tail of rare events.

%If $\mathcal{P}_N$ denotes the probability of sampling a novel (previously unseen) event from some distribution after having sampled $N$ events, then productivity as described above states that $\mathcal{P}_N > 0$ for all sample sizes $N$ that occur in practice.

\paragraph{LNRE Zone} To make explicit the connection between productivity and a heavy-tail of rare events, let $\mathcal{P}_N$ denote the probability of
sampling a novel (previously unseen) event from some distribution
after having sampled $N$ events. Then productivity as described above
states that $\mathcal{P}_N > 0$ for all sample sizes $N$ that occur in
practice. The range of sample sizes $N$ for which it is the case that
$\mathcal{P}_N > 0$ is known as the \textsl{LNRE zone}
\citep{Khmaladze1988TheSA, Baayen2001WordFD}. The LNRE zone for
natural language appears to be very large, and it seems likely that
$\mathcal{P}_N$ will remain greater than $0$ for samples of natural
language many orders of magnitude larger than all the data currently
available for training LMs.\footnote{For an empirical validation of
  this claim on a sample of practical size from the OpenWebText
  corpus, see the Appendix.}  In the LNRE zone, it is difficult
to obtain accurate estimates of the probability of events using
straightforward maximum likelihood estimation (MLE). Accounting for this enormous amount of
novelty is thus a central challenge in language modeling.

\paragraph{Language modeling} 
%A model $M$ of the language $L$ attempts to define a distribution $p_M$ over variable length sequences $\vx = (x_1, \dots, x_{|\vx|})$ which closely resembles the true distribution of the language $p_L$. That is,~$p_M(\vx) \approx p_L(\vx) \text{ for all } \vx \in \Sigma^*$, where $\Sigma$ denotes the vocabulary of $M$, and $\Sigma^*$ is the set of all strings of finite length, known as the Kleene closure of $\Sigma$. 

A model $M$ of the language $L$ attempts to define a distribution $p_M$ which closely resembles the true distribution of the language $p_L$. In a locally-normalized autoregressive model, this distribution is defined by assigning probabilities to variable length sequences $\vx$ via a chain-rule decomposition:

\begin{equation}
    p(\vx) = \prod_{i=1}^{|\vx|} p(x_i \mid \vx_{1:i-1})
    = \prod_{i=1}^{|\vx|} \frac{\exp \rho(\vx_{1:i-1}, x_i) }{\sum_{x \in \Sigma} \exp \rho(\vx_{1:i-1}, x) }
\end{equation}

where $\Sigma$ is the vocabulary, and $\rho(\vx_{1:i-1}, x_i; \theta)$ is the non-negative score of token $x_i$ given the sequence prefix $\vx_{1:i-1}$, which is computed by a neural network with parameters $\theta$.

For $p_M$ to perfectly approximate $p_L$, we expect~$p_M(\vx) = p_L(\vx) \text{ for all } \vx \in \Sigma^*$, where $\Sigma^*$ is the set of all strings of finite length (the Kleene closure of $\Sigma$).  In the LNRE zone, $p_M$ is defined over a support containing a very large set of sequences which have never occurred in a training corpus (or equivalently, have all occurred with frequency $0$), and which take on a very wide array of differing probabilities. For example, while the sequences $\vx_1, \vx_2 \in \Sigma^*$ have likely never occurred in any sample of English, most would agree that $\vx_1$ is far more probable than $\vx_2$:
\begin{itemize}
\item [$\vx_1$:] \emph{The East pond in Parc Lafontaine was filled to the brim with Diet Coke.}
\item [$\vx_2$:] \emph{Certain nak indicate liberationing among theorter codity voters vandalized.}
\end{itemize}

%Traditional $n$-gram models attempted to increase the reliability of frequency-based estimation by assuming that the probability of a word depends only on a finite context (typically 2-3 words). By exponentially reducing the number of outcomes to be estimated, this Markov assumption made it possible to compute semi-reliable relative frequencies from large corpora. However, because of the number of rare events, these estimates still did not converge to their population probabilities, and had to be adjusted using \textsl{smoothing} methods \citep{Jelinek1980InterpolatedEO, katz, kneser-ney}. 

%Autoregressive neural language models attempt to overcome the challenges of the LNRE zone using a neural-parameterized chain rule decomposition. Specifically, a sequence $\vx$ is assigned a probability according to its chain rule decomposition, with each conditional distribution parameterized by a model $M$, where $M$ jointly learns a set of real-valued distributed feature vectors and the parameters of the probability function $p_M$ by minimizing the negative log-likelihood of a set of samples $\mathcal{D}$ drawn from $L$.


\paragraph{LM Evaluation} For a perfect LM of English, we would expect
the estimated probabilities of the sequences $\vx_1$ and $\vx_2$ to
match their probabilities under the true distribution
$p_\text{English}$. However, since $p_\text{English}$ and it's
underlying generative process are unknown, it is not possible to
explicitly evaluate how closely instance-level probability estimates
align. As a proxy, the mean perplexity of the model on a holdout set
of sequences $\mathcal{D}$ is typically used, %:
%\begin{equation}\label{eq:perp}\small
%    PP(p_M, \mathcal{D}) = \frac{1}{|\mathcal{D}|}\sum_{i=1}^{|\mathcal{D}|} \exp{\left\{-\frac{1}{|\vx^{(i)} |}\sum_{t=1}^{|\vx^{(i)} |} \log p_M(x_t^{(i)} \mid x_{<t}^{(i)})\right\}}
%\end{equation}
which measures whether the model, on average, assigns high likelihood
to unseen instances. This measure does not, however, tell us whether
instance-level estimates align with their true counterparts, nor is
it necessarily indicative of performance on rare, idiosyncratic events
in $\mathcal{D}$. In this way, the lack of access to the
ground-truth distribution severely complicates LM evaluation on the
heavy-tail of rare sequences in language. The following section introduces a methodology to overcome these limitations.


==> LMs and Syntactic Complexity/SEC_background_old.tex <==
In this section, we briefly characterize why distributions with a large number of rare events (LNRE) emerge in natural language, and why these events pose challenges for models of natural language. Furthermore, we motivate the need for instance-level evaluation when dealing with a large number of rare events.

%\tjo{I think the LNRE zone discussion below needs a bit more unpacking. It could go by fast for a reader who wasn't watching out for it.}

\paragraph{Productivity}
In the context of language production, at any given point in their linguistic lifespan, a language user has the ability to produce an utterance which they have never produced before. This is the result of the generative property of \textsl{productivity},  which states that on the basis of finite linguistic experience, a language user can produce and comprehend an unbounded number of grammatically acceptable utterances \citep{chomsky1979logical}\alex{change to 1975}.
% LNRE distributions in language emerge as a result of the generative property of \textsl{productivity}. Productivity states that on the basis of finite linguistic experience, a language user can produce and comprehend an unbounded number of grammatically acceptable utterances \citep{chomsky1979logical} [change to 1975].\tjo{this is also a side effect of productivity, productivity just means that the speaker can say and understand new things. This is in practice unbounded.}
% In the context of language production, for example, this means that at any given point in their linguistic lifespan, a language user has the ability to produce an utterance which they have never produced before.\tjo{right, so this paragraph is backwards for me.}

% LNRE distributions in language emerge as a result of the generative property of \textsl{productivity}. Productivity states that on the basis of finite linguistic experience, a language user can produce and comprehend an unbounded number of grammatically acceptable utterances \citep{chomsky1979logical} [change to 1975].\tjo{this is also a side effect of productivity, productivity just means that the speaker can say and understand new things. This is in practice unbounded.}
% In the context of language production, for example, this means that at any given point in their linguistic lifespan, a language user has the ability to produce an utterance which they have never produced before.\tjo{right, so this paragraph is backwards for me.}

\begin{wrapfigure}{r}{0.5\textwidth}
\centering
\includegraphics[width=0.3\textwidth]{figures/lnre-ex-bars-2.png}
\caption{\small Productivity $\mathcal{P}$ as a function of sample
  size $N$. Distributions in natural language are characterized by a
  potentially unbounded amount of novelty. [make plot readable]}
\label{fig:lnre-ex}
\end{wrapfigure}

Because of its productivity, distributions in language consist of a large number of rare events. Let $\mathcal{P}_N$ denote the probability
of sampling a novel (previously unseen) event from some distribution
after having sampled $N$ events. This quantity can be interpreted as
the amount of probability mass the distribution places on unseen
events after $N$ samples. Productivity, as stated above, says that
$\mathcal{P}_N > 0$ for all $N$. A productive process
induces a distribution which places non-zero probability on unseen
events, no matter how large the sample size.\footnote{For a more
  precise formulation of this definition, due to
  \cite{Khmaladze1988TheSA}, as well as a frequentist estimator for
  $\mathcal{P}_N$, see the Appendix.}

\paragraph{LNRE Zone} The range of sample sizes $N$ for which it is the case that $\mathcal{P}_N > 0$ is known as the \textsl{LNRE zone} \citep{Baayen2001WordFD}. Crucially, in the case of the distribution over the
sequences of a language, for any
practical sample size, unseen events will account for a non-negligible amount of the total probability mass of the distribution.\tjo{I feel
  like we can state this more clearly and more strongly. I wouldn't
  just say practical, i would talk about orders of magnitude of data
  involved being larger than all the data ever collected by humans or
  whatever.} For an empirical validation of the claim, see Figure
\ref{fig:lnre-ex}.

% We empirically validate this claim on OpenWebText, a popular
% language modeling corpus. In Figure \ref{fig:lnre-ex}, we plot the
% the empirical estimate of $\mathcal{P}$ as function of the sample
% size $N$ for sentences and trigrams sampled from a subset of
% OpenWebText. For comparison, we also include the potential
% productivity of two fair dice (uniform multinomial distributions),
% with increasingly large support. Whereas $\mathcal{P}$ quickly
% decreases to 0 in the case of fair dice, in the OpenWebText
% distributions, there is very high probability of observing a novel
% event, even for large $N$.\alex{maybe cut}

When distributions place non-negligible probability on unseen
outcomes, it is not possible to estimate the probability of events
using a straightforward maximum likelihood estimate (MLE). \tjo{this
  needs a citation and some sort of brief explanation. Surely if this
  is known, it is known outside of baayen's weird little world. Like
  the literature on Good Turing must say something about
  this.} If unobserved events have a non-negligible amount of probability mass for all practical sample sizes, then the sample relative frequencies of observed events will fail to converge to their population probabilities. The LNRE zone can thus be thought of as the range of sample sizes in
which relative frequencies cannot be trusted to converge to their population probabilities.\footnote{By failing to set aside probability for unseen events, the sample relative frequencies of observed events will necessarily overestimate their population probabilities.}

 %Since distributions in the LNRE zone place non-negligible probability on unseen outcomes, it is not possible to estimate the probability of events using a straightforward maximum likelihood estimate (MLE). A typical MLE  for the probability of an event is its relative frequency in some sample of sufficient size $N$. However, if unobserved events have a non-negligible amount of probability mass for all practical values of $N$, then the sample relative frequencies of observed events will fail to converge to their population probabilities.\footnote{To see this, note that by failing to set aside probability for unseen events, the sample relative frequencies of observed events will necessarily overestimate their population probabilities.}  

\paragraph{Language modeling} 

Accounting for the potentially unbounded amount of novelty in the LNRE zone is one of the fundamental challenges in language modeling. A model $M$ of the language $L$ attempts to define a distribution $p_M$ over variable length sequences $\vx = (x_1, \dots, x_{|\vx|})$ which closely resembles the true distribution of the language $p_L$, that is,~$p_M(\vx) \approx p_L(\vx) \text{ for all } \vx \in \Sigma^*$, where $\Sigma$ denotes the vocabulary of $M$, and $\Sigma^*$ is the set of all strings of finite length, known as the Kleene closure of $\Sigma$.

%What is so difficult about the LNRE zone is not only that any practical sample size will exclude a large number of events, but also that this set each of the outcomes in this set will of unseen outcomes will 

In the LNRE zone, any sample of practical size from $p_L$ will exclude
the majority of possible outcomes in $\Sigma^*$. A LM must therefore define a distribution over a support containing a
large set of sequences which have never occurred in a training corpus
(or equivalently, have all occurred with frequency $0$), yet each take
on vastly different probabilities. For example, while the sequences
$\vx_1, \vx_2 \in \Sigma^*$ have likely never occurred in any sample
of English, most would agree that $\vx_1$ is far more probable than
$\vx_2$.
\begin{itemize}
\item [$\vx_1$:] \emph{The East pond in Parc Lafontaine was filled to the brim with diet Coke.}
\item [$\vx_2$:] \emph{Certain nak indicate liberationing among theorter codity voters vandalized.}
\end{itemize}

%Traditional $n$-gram models attempted to increase the reliability of frequency-based estimation by assuming that the probability of a word depends only on a finite context (typically 2-3 words). By exponentially reducing the number of outcomes to be estimated, this Markov assumption made it possible to compute semi-reliable relative frequencies from large corpora. However, because of the number of rare events, these estimates still did not converge to their population probabilities, and had to be adjusted using \textsl{smoothing} methods \citep{Jelinek1980InterpolatedEO, katz, kneser-ney}. 

%Autoregressive neural language models attempt to overcome the challenges of the LNRE zone using a neural-parameterized chain rule decomposition. Specifically, a sequence $\vx$ is assigned a probability according to its chain rule decomposition, with each conditional distribution parameterized by a model $M$, where $M$ jointly learns a set of real-valued distributed feature vectors and the parameters of the probability function $p_M$ by minimizing the negative log-likelihood of a set of samples $\mathcal{D}$ drawn from $L$.

\paragraph{Perplexity} A perfect model $M$ of the language $L$ defines a distribution $p_M$ which assigns the same probability to all strings in $\Sigma^*$ as the true distribution of the language $p_L$. Since $p_L$ and the underlying generative process are in practice unknown, it is not possible to explicitly
evaluate how closely these distributions align. As a proxy, the mean perplexity of the model on a withheld set of sequences $\mathcal{D}^\prime$ is typically used:
\begin{equation}\label{eq:perp}
    PP(p_M, \mathcal{D}^\prime) = \frac{1}{|\mathcal{D}^\prime|}\sum_{i=1}^{|\mathcal{D}^\prime|} \exp{\left\{-\frac{1}{|\vx^{(i)} |}\sum_{t=1}^{|\vx^{(i)} |} \log p_M(x_t^{(i)} \mid x_{<t}^{(i)})\right\}}
\end{equation}

Perplexity therefore measures whether the model, on average, assigns high likelihood to
unseen instances. It does not, however, tell us whether instance-level estimations align with their true counterparts, nor is it necessarily indicative of performance on held-out rare events. In this way, without knowledge of instance-level probability estimation performance, it is difficult to conduct an in-depth analysis of LM performance in the heavy-tail of rare events of the distribution. In the following section, we propose a methodology to overcome these shortcomings. 

==> LMs and Syntactic Complexity/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> SEC_background_old.tex <==
In this section, we briefly characterize why distributions with a large number of rare events (LNRE) emerge in natural language, and why these events pose challenges for models of natural language. Furthermore, we motivate the need for instance-level evaluation when dealing with a large number of rare events.

%\tjo{I think the LNRE zone discussion below needs a bit more unpacking. It could go by fast for a reader who wasn't watching out for it.}

\paragraph{Productivity}
In the context of language production, at any given point in their linguistic lifespan, a language user has the ability to produce an utterance which they have never produced before. This is the result of the generative property of \textsl{productivity},  which states that on the basis of finite linguistic experience, a language user can produce and comprehend an unbounded number of grammatically acceptable utterances \citep{chomsky1979logical}\alex{change to 1975}.
% LNRE distributions in language emerge as a result of the generative property of \textsl{productivity}. Productivity states that on the basis of finite linguistic experience, a language user can produce and comprehend an unbounded number of grammatically acceptable utterances \citep{chomsky1979logical} [change to 1975].\tjo{this is also a side effect of productivity, productivity just means that the speaker can say and understand new things. This is in practice unbounded.}
% In the context of language production, for example, this means that at any given point in their linguistic lifespan, a language user has the ability to produce an utterance which they have never produced before.\tjo{right, so this paragraph is backwards for me.}

% LNRE distributions in language emerge as a result of the generative property of \textsl{productivity}. Productivity states that on the basis of finite linguistic experience, a language user can produce and comprehend an unbounded number of grammatically acceptable utterances \citep{chomsky1979logical} [change to 1975].\tjo{this is also a side effect of productivity, productivity just means that the speaker can say and understand new things. This is in practice unbounded.}
% In the context of language production, for example, this means that at any given point in their linguistic lifespan, a language user has the ability to produce an utterance which they have never produced before.\tjo{right, so this paragraph is backwards for me.}

\begin{wrapfigure}{r}{0.5\textwidth}
\centering
\includegraphics[width=0.3\textwidth]{figures/lnre-ex-bars-2.png}
\caption{\small Productivity $\mathcal{P}$ as a function of sample
  size $N$. Distributions in natural language are characterized by a
  potentially unbounded amount of novelty. [make plot readable]}
\label{fig:lnre-ex}
\end{wrapfigure}

Because of its productivity, distributions in language consist of a large number of rare events. Let $\mathcal{P}_N$ denote the probability
of sampling a novel (previously unseen) event from some distribution
after having sampled $N$ events. This quantity can be interpreted as
the amount of probability mass the distribution places on unseen
events after $N$ samples. Productivity, as stated above, says that
$\mathcal{P}_N > 0$ for all $N$. A productive process
induces a distribution which places non-zero probability on unseen
events, no matter how large the sample size.\footnote{For a more
  precise formulation of this definition, due to
  \cite{Khmaladze1988TheSA}, as well as a frequentist estimator for
  $\mathcal{P}_N$, see the Appendix.}

\paragraph{LNRE Zone} The range of sample sizes $N$ for which it is the case that $\mathcal{P}_N > 0$ is known as the \textsl{LNRE zone} \citep{Baayen2001WordFD}. Crucially, in the case of the distribution over the
sequences of a language, for any
practical sample size, unseen events will account for a non-negligible amount of the total probability mass of the distribution.\tjo{I feel
  like we can state this more clearly and more strongly. I wouldn't
  just say practical, i would talk about orders of magnitude of data
  involved being larger than all the data ever collected by humans or
  whatever.} For an empirical validation of the claim, see Figure
\ref{fig:lnre-ex}.

% We empirically validate this claim on OpenWebText, a popular
% language modeling corpus. In Figure \ref{fig:lnre-ex}, we plot the
% the empirical estimate of $\mathcal{P}$ as function of the sample
% size $N$ for sentences and trigrams sampled from a subset of
% OpenWebText. For comparison, we also include the potential
% productivity of two fair dice (uniform multinomial distributions),
% with increasingly large support. Whereas $\mathcal{P}$ quickly
% decreases to 0 in the case of fair dice, in the OpenWebText
% distributions, there is very high probability of observing a novel
% event, even for large $N$.\alex{maybe cut}

When distributions place non-negligible probability on unseen
outcomes, it is not possible to estimate the probability of events
using a straightforward maximum likelihood estimate (MLE). \tjo{this
  needs a citation and some sort of brief explanation. Surely if this
  is known, it is known outside of baayen's weird little world. Like
  the literature on Good Turing must say something about
  this.} If unobserved events have a non-negligible amount of probability mass for all practical sample sizes, then the sample relative frequencies of observed events will fail to converge to their population probabilities. The LNRE zone can thus be thought of as the range of sample sizes in
which relative frequencies cannot be trusted to converge to their population probabilities.\footnote{By failing to set aside probability for unseen events, the sample relative frequencies of observed events will necessarily overestimate their population probabilities.}

 %Since distributions in the LNRE zone place non-negligible probability on unseen outcomes, it is not possible to estimate the probability of events using a straightforward maximum likelihood estimate (MLE). A typical MLE  for the probability of an event is its relative frequency in some sample of sufficient size $N$. However, if unobserved events have a non-negligible amount of probability mass for all practical values of $N$, then the sample relative frequencies of observed events will fail to converge to their population probabilities.\footnote{To see this, note that by failing to set aside probability for unseen events, the sample relative frequencies of observed events will necessarily overestimate their population probabilities.}  

\paragraph{Language modeling} 

Accounting for the potentially unbounded amount of novelty in the LNRE zone is one of the fundamental challenges in language modeling. A model $M$ of the language $L$ attempts to define a distribution $p_M$ over variable length sequences $\vx = (x_1, \dots, x_{|\vx|})$ which closely resembles the true distribution of the language $p_L$, that is,~$p_M(\vx) \approx p_L(\vx) \text{ for all } \vx \in \Sigma^*$, where $\Sigma$ denotes the vocabulary of $M$, and $\Sigma^*$ is the set of all strings of finite length, known as the Kleene closure of $\Sigma$.

%What is so difficult about the LNRE zone is not only that any practical sample size will exclude a large number of events, but also that this set each of the outcomes in this set will of unseen outcomes will 

In the LNRE zone, any sample of practical size from $p_L$ will exclude
the majority of possible outcomes in $\Sigma^*$. A LM must therefore define a distribution over a support containing a
large set of sequences which have never occurred in a training corpus
(or equivalently, have all occurred with frequency $0$), yet each take
on vastly different probabilities. For example, while the sequences
$\vx_1, \vx_2 \in \Sigma^*$ have likely never occurred in any sample
of English, most would agree that $\vx_1$ is far more probable than
$\vx_2$.
\begin{itemize}
\item [$\vx_1$:] \emph{The East pond in Parc Lafontaine was filled to the brim with diet Coke.}
\item [$\vx_2$:] \emph{Certain nak indicate liberationing among theorter codity voters vandalized.}
\end{itemize}

%Traditional $n$-gram models attempted to increase the reliability of frequency-based estimation by assuming that the probability of a word depends only on a finite context (typically 2-3 words). By exponentially reducing the number of outcomes to be estimated, this Markov assumption made it possible to compute semi-reliable relative frequencies from large corpora. However, because of the number of rare events, these estimates still did not converge to their population probabilities, and had to be adjusted using \textsl{smoothing} methods \citep{Jelinek1980InterpolatedEO, katz, kneser-ney}. 

%Autoregressive neural language models attempt to overcome the challenges of the LNRE zone using a neural-parameterized chain rule decomposition. Specifically, a sequence $\vx$ is assigned a probability according to its chain rule decomposition, with each conditional distribution parameterized by a model $M$, where $M$ jointly learns a set of real-valued distributed feature vectors and the parameters of the probability function $p_M$ by minimizing the negative log-likelihood of a set of samples $\mathcal{D}$ drawn from $L$.

\paragraph{Perplexity} A perfect model $M$ of the language $L$ defines a distribution $p_M$ which assigns the same probability to all strings in $\Sigma^*$ as the true distribution of the language $p_L$. Since $p_L$ and the underlying generative process are in practice unknown, it is not possible to explicitly
evaluate how closely these distributions align. As a proxy, the mean perplexity of the model on a withheld set of sequences $\mathcal{D}^\prime$ is typically used:
\begin{equation}\label{eq:perp}
    PP(p_M, \mathcal{D}^\prime) = \frac{1}{|\mathcal{D}^\prime|}\sum_{i=1}^{|\mathcal{D}^\prime|} \exp{\left\{-\frac{1}{|\vx^{(i)} |}\sum_{t=1}^{|\vx^{(i)} |} \log p_M(x_t^{(i)} \mid x_{<t}^{(i)})\right\}}
\end{equation}

Perplexity therefore measures whether the model, on average, assigns high likelihood to
unseen instances. It does not, however, tell us whether instance-level estimations align with their true counterparts, nor is it necessarily indicative of performance on held-out rare events. In this way, without knowledge of instance-level probability estimation performance, it is difficult to conduct an in-depth analysis of LM performance in the heavy-tail of rare events of the distribution. In the following section, we propose a methodology to overcome these shortcomings. 
